Phase Semantic Cut-elimination for Intuitionistic Linear Logic with Least and Greatest Fixed Points

This paper establishes the cut-elimination theorem for intuitionistic propositional multiplicative-additive linear logic with the least and greatest fixpoints ($\mu$IMALL) by means of its phase semantics. A classical first-order multiplicative-additive linear logic system with the least and greatest fixpoints was introduced by Baelde and Miller (2007). Its intuitionistic fragment was discussed in Baelde (2012), but the cut-elimination theorem for this fragment has not yet been proved. We introduce a propositional fragment of this system, $\mu$IMALL, and establish the cut-elimination theorem. To prove the theorem, we define phase semantics for $\mu$IMALL and show the following two statements: (1) Soundness: if a formula is provable in $\mu$IMALL, then it is true in all phase models, and (2) Cut-free Completeness: if a formula is true in all phase models, then it is provable in $\mu$IMALL without Cut. Okada (1999, 2002) employed a phase semantic method to prove the cut-elimination theorems for classical and intuitionistic linear logic systems. De et al. (2022) applied this method to a propositional fragment of classical propositional multiplicative-additive linear logic with the least and greatest fixpoints. We refine and apply their arguments to prove the cut-elimination theorem for $\mu$IMALL.

==> eptcsdata.tex <==
\providecommand{\firstpage}{221}
\providecommand{\publicationstatus}{V. de Paiva; T.A. de Lima (Eds.): 21st International Symposium\\ on Logical and Semantic Frameworks, with Applications (LSFA 2026)\\
EPTCS 449, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.449.14}{10.4204/EPTCS.449.14}}

